A Systematic Literature Review on Explainability for Machine/Deep Learning-based Software Engineering Research

The remarkable achievements of Artificial Intelligence (AI) algorithms, particularly in Machine Learning (ML) and Deep Learning (DL), have fueled their extensive deployment across multiple sectors, including Software Engineering (SE). However, due to their black-box nature, these promising AI-driven SE models are still far from being deployed in practice. This lack of explainability poses unwanted risks for their applications in critical tasks, such as vulnerability detection, where decision-making transparency is of paramount importance. This paper endeavors to elucidate this interdisciplinary domain by presenting a systematic literature review of approaches that aim to improve the explainability of AI models within the context of SE. The review canvasses work appearing in the most prominent SE & AI conferences and journals, and spans 108 papers across 23 unique SE tasks. Based on three key Research Questions (RQs), we aim to (1) summarize the SE tasks where XAI techniques have shown success to date; (2) classify and analyze different XAI techniques; and (3) investigate existing evaluation approaches. Based on our findings, we identified a set of challenges remaining to be addressed in existing studies, together with a set of guidelines highlighting potential opportunities we deemed appropriate and important for future work.

==> language.tex <==
\section{Analysis Policy Language}
\label{sec:language}

This section introduces the syntax of the analysis policy language (\cref{subsec:syntax}) and two important relations (\cref{subsec:sr}). 
Lastly, we formulate a static analysis problem as the analysis policy evaluation (\cref{subsec:pf}).
% that facilitates describing the decomposition of a static analysis problem. 
% We first introduce the syntax of the analysis policy language (\cref{subsec:syntax}) and then detail two important relations used in the language, namely symbolic and neural relations (\cref{subsec:sr}). Lastly we formulate a static analysis problem as the analysis policy evaluation (\cref{subsec:pf}).

\subsection{Syntax}
\label{subsec:syntax}

\begin{comment}
\begin{figure}[t]
\footnotesize
\centering
\[
\begin{aligned}
    \text{Analysis Policy} \quad  &p ::= r_1 \mid r_2 \mid \dots \mid r_n \\
    \text{Rule} \quad             &r ::= R_I \leftarrow R_1, R_2, \dots, R_n \\
    \text{Relation} \quad         &R ::= R_S \mid R_N \mid R_I \\
    \text{Symbolic Relation} \quad    &R_S ::= R_S(a_1) \mid R_S(a_1, a_2) \\
    \text{Neural Relation} \quad      &R_N ::= R_N(a_1) \mid R_N(a_1, a_2) \\
    \text{Intensional Relation} \quad &R_I ::= R_I(a_1) \mid R_I(a_1, a_2) \\
    \text{Term} \quad & a \in \textsf{Dom} ::= \textsf{Expr} \cup \textsf{String} \cup \textsf{Int}
\end{aligned}
\]
\vspace{-2mm}
\caption{The syntax of the analysis policy language}
\vspace{-2mm}
\label{fig:syntax}
\end{figure}
\end{comment}

\begin{comment}
The essential of a static analysis problem is to compute a specific relation depicting desired program properties.
For example, program slicing computes a binary relation $R_{\textsf{slice}} = \{(e, \ell)\}$ such that the value of the expression $e$ in the slicing seed depends on the execution of the statement at line $\ell$.
Similarly, typical bug detection, such as taint-style bug detection, can be reduced to computing the relation $R_{\textsf{taint}} = \{(e_{src}, e_{sink})\}$ that indicates the tainted value of expression $e_{src}$  affects the value of the argument $e_{sink}$ at some critical function.
Notably, a relation depicting a complex program property can be derived from multiple relations describing simpler program properties.
For instance, a program slice can be determined according to the data and control dependencies.
Hence, we can solve a sophisticated static analysis problem via divide-and-conquer,
i.e., by decomposing the original analysis problem and composing the relations obtained in solving the sub-problems.\xz{redundancy again}
\end{comment}

\begin{wrapfigure}[9]{r}{0.5\textwidth}
	%\begin{wrapfigure}[13]{r}{0.52\textwidth}
	%\vspace{-6mm}
	\vspace{-10mm}
	\centering
	\scalebox{1.0}{
		\begin{minipage}{0.51\textwidth}
			\centering
            \begin{figure}[H]
                \footnotesize
                \centering
                \[
                \begin{aligned}
                    \text{Analysis Policy} \quad  &p ::= r_1 \mid r_2 \mid \dots \mid r_n \\
                    \text{Rule} \quad             &r ::= R_I \leftarrow R_1, R_2, \dots, R_n \\
                    \text{Relation} \quad         &R ::= R_S \mid R_N \mid R_I \\
                    \text{Symbolic Relation} \quad    &R_S ::= R_S(a_1) \mid R_S(a_1, a_2) \\
                    \text{Neural Relation} \quad      &R_N ::= R_N(a_1) \mid R_N(a_1, a_2) \\
                    \text{Intensional Relation} \quad &R_I ::= R_I(a_1) \mid R_I(a_1, a_2) \\
                    \text{Term} \quad & a \in \textsf{Dom} ::= \textsf{Expr} \cup \textsf{String} \cup \textsf{Int}
                \end{aligned}
                \]
                \vspace{-2mm}
                \caption{The syntax of the analysis policy language}
                \vspace{-2mm}
                \label{fig:syntax}
                \end{figure}
		\end{minipage}
	}
\end{wrapfigure}
The essential of a static analysis problem is to compute a specific relation depicting desired program properties.
As demonstrated in~\cref{subsubsec:approach}, a static analysis problem can be decomposed into several sub-problems targeting simpler properties.
Utilizing the relations depicting the properties targeted in the sub-problems, we can derive the desired property to achieve the original analysis goal.


Based on the above insight, we adopt Datalog as our analysis policy language that supports the users in specifying the problem decomposition.
The syntax of the analysis policy language is formulated in Figure~\ref{fig:syntax}.
Specifically, \emph{an analysis policy is a set of Datalog rules that solve a specific static analysis problem via divide-by-conquer.}
Each Datalog rule derives a specific relation in its \emph{head} (i.e., its left hand), namely an \emph{intensional relation}, from the relations in its \emph{body} (i.e., its right hand). 
%\shi{why not a definition for analysis policy/head/body}\wcp{Seem unnecessary. Quite basic concepts. I just want to briefly introduce them without explicit definitions.}
Unlike traditional Datalog programs,
we introduce \emph{symbolic} and \emph{neural} relations depicting syntactic and semantic program properties, respectively,
which can only appear in the body of a rule.
An \emph{output relation} is defined as a relation that does not occur within the body of any rule in the analysis policy except within rules that derive the relation itself.
Actually, it indicates the program property targeted in the original static analysis problem.
Since most common program properties can be formulated by unary and binary relations,
we only permit unary and binary relations in the analysis policy, which have one and two terms, respectively.
Our work concentrates on expression-related properties,
and thus, the domain of the terms in relations is set to contain expressions, string values, and integer values.
Here, string values can encode the string representations of expressions,
while integer values indicate program lines.
Without the loss of expressiveness, we restrict the number of neural relations in the rule to be at most one.
Other rules can be transformed into multiple rules conforming to our syntax by introducing several intermediate intensional relations.



\begin{example}\xz{I see you introduce the details of the Figure 4 rules only here. Then you may want to re-org your text. In the last section, you mention Fig 4 without discussing it. You want the readers to figure them out? If they already figure them out earlier, why they need to read the following. And it seems that you do need to mention Figure 4 earlier because your discussion in 2.2.2 indeed requires talking about them.}\xz{I think the main problem of the writing lies in the arrangement of information, especially which parts should be more abstract, more concrete, instead of repeating the same thing again and again.}
	Figure~\ref{fig:input} shows the analysis policy of program slicing. The rules (2) and (3) collect direct data and control dependencies of the slicing seed, respectively. Rules (4) and (5) transitively collect the data and control dependencies of the expressions on which the slicing seed depends, respectively. Finally, the output relation \textsf{Slice} is derived by the rule (1), depicting all the program lines belonging to the desired program slice.
	Similarly, in Figure~\ref{fig:xss-rules}, the detection of intra-procedural XSS bugs is decomposed into the sub-problems of identifying sources/sinks (formulated by rules (2) and (3)) and determining intra-procedural taint flows between expressions (formulated by rule (1)).
	%Specifically, the sources and sinks are depicted by the unary neural relations \textsf{XSSSrcNeural} and \textsf{XSSSinkNeural},
	%while the binary neural relation maintains intra-procedural taint flows. 
\end{example}



\subsection{Symbolic and Neural Relation}
\label{subsec:sr}

%\shi{it seems we can merge 3.1 \& 3.2 into subsection 3.1, consisting of three subsubsections for analysis policy, symbolic relation, and neural relation, respectively?}\wcp{I prefer not. Section 3.1 defines the syntax, while Section 3.2 presents the semantics of different symbolic relations and how to specify the semantics of neural relations with neural relation specifications.}

As demonstrated by Figure~\ref{fig:syntax} in~\cref{subsec:syntax},
symbolic and neural relations are the basis of the analysis,
depicting syntactic and semantic properties as prerequisites.
In what follows, we will provide further details on the two kinds of relations.

\subsubsection{Symbolic Relation}
In static analysis, we basically focus on the properties of specific program constructs. For instance, specific expressions, including those associated with specific names or located at specific lines, function parameters/return values, and arguments/output values at function call sites, are often the pivot constructs that facilitate the analysis. Besides, program properties relating to control flows, such as control-flow order and control dependencies, are also required in many static analysis applications. These program properties can be directly obtained through parsing the AST of a program, offering broad applicability across various static analysis tasks.

To support the customization, we introduce a set of symbolic relations shown in Table~\ref{tab:symbolic-relation-syntax} to depict common syntactic properties.
% Sepecifically, we pre-define relations to depict properties, including function arguments (\textsf{Args}), function outputs (\textsf{Outs}), parameters (\textsf{Paras}) and return values (\textsf{Rets}), expression names (\textsf{ExprName}) and locations (\textsf{ExprLoc}), and control-flow order (\textsf{CtrlOrd}) and control dependency (\textsf{CtrlDep}). 
% To support inter-procedural analysis, we introduce the relations \textsf{ArgPara} and \textsf{OutRet}
% that match the arguments and outputs of function calls with the parameters and return values of callee functions, respectively.
Specifically, the relations \textsf{Args} and \textsf{Outs} maintain the arguments and outputs of function calls, respectively,
while the relations \textsf{Paras} and \textsf{Rets} maintain the parameters and return values of functions, respectively.
To localize specific expressions, we offer two relations, namely \textsf{ExprName} and \textsf{ExprLoc}, that maintain the expressions along with their names and program lines, respectively.
We also introduce the relations \textsf{CtrlOrd} and 
\textsf{CtrlDep} to maintain the control-flow order and 
control dependency between different expressions.
To support inter-procedural analysis, we introduce the relations \textsf{ArgPara} and \textsf{OutRet}
that match the arguments and outputs of function calls with the parameters and return values of callee functions, respectively.
\xz{this simple formulation makes me think about (context) sensitivity. You may need to discuss that if you haven't done so}\wcp{revised}
Our work does not consider calling contexts and only facilitates the context-insensitive analysis.
\wcp{To be discussed at the end of the evaluation. Future work.}

\begin{comment}
Basically, symbolic relations can be efficiently derived from ASTs of the program after parsing.
When computing the symbolic relations \textsf{ArgPara}, \textsf{OutRet}, and \textsf{caller\_callee}, we do not consider advance language features, such as reflections and function pointers,
and instead, only leverage syntactic properties, such as the function type signatures, to approximate the call graph.
\end{comment}

\begin{table}[t]
	\centering
	\caption{Symbolic relations and their descriptions}
	\footnotesize
	\begin{tabular}{p{0.08\textwidth} p{0.25\textwidth} p{0.58\textwidth}}
		\toprule
		\textbf{Arity} & \textbf{Symbolic Relation} & \textbf{Description} \\ \midrule
		Unary & \textsf{Args(e:Expr)} & Argument $\textsf{e}$ of a function call \\
		Unary & \textsf{Outs(e:Expr)} & Output $\textsf{e}$ of a function call \\
		Unary & \textsf{Paras(e:Expr)} & Parameter $\textsf{e}$ of a function \\
		Unary & \textsf{Rets(e:Expr)} & Return value $\textsf{e}$ of a function \\
		Unary & \textsf{ExprName(e:Expr, s:String)} & Expression $\textsf{e}$ with name $s$ \\
		Unary & \textsf{ExprLoc(e:Expr, $l$:Int)} & Expression $\textsf{e}$ at line $l$ \\ \midrule
		Binary & \textsf{CtrlOrd(\textsf{e1}:Expr, \textsf{e2}:Expr)} & The expression $\textsf{e1}$ may be evaluated before $\textsf{e2}$ in a single function \\
		Binary & \textsf{CtrlDep(\textsf{e1}:Expr, \textsf{e2}:Expr)} & The value of $\textsf{e1}$ affects whether $\textsf{e2}$ is evaluated or not in a single function \\
		Binary & \textsf{ArgPara(\textsf{e1}:Expr, \textsf{e2}:Expr)} & Arguments of function calls $\textsf{e1}$ match with parameters $\textsf{e2}$ \\
		Binary & \textsf{OutRet(\textsf{e1}:Expr, \textsf{e2}:Expr)} & Output of function calls $\textsf{e1}$ matches with return values $\textsf{e2}$ \\ \bottomrule
	\end{tabular}
	\label{tab:symbolic-relation-syntax}
	\vspace{-3mm}
\end{table}

\begin{figure}[t]
	\centering
	\footnotesize
 %\vspace{-3mm}
	\begin{align}
		\textsf{XSSBug}(\textsf{e1}, \textsf{e2}) & \leftarrow \textsf{XSSSrc}(\textsf{e1}), \textsf{\color{red}{TaintProp}}(\textsf{e1}, \textsf{e2}), \textsf{XSSSink}(\textsf{e2})\\
		\textsf{XSSSrc}(\textsf{e1}) &\leftarrow \textsf{\color{red}{XSSSrcNeural}}(\textsf{e1})\\
		\textsf{XSSSink}(\textsf{e1}) &\leftarrow \textsf{\color{red}{XSSSinkNeural}}(\textsf{e1})
	\end{align}
    %\vspace{-2mm}
	\caption{An analysis policy of intra-procedural XSS detection. The neural relations are in {\color{red}{red}}.}
 %\vspace{-5mm}
	\label{fig:xss-rules}
\end{figure}

\begin{example}
As shown in Figure~\ref{fig:input}(a), the symbolic relations  \textsf{ExprName} and \textsf{ExprLoc} 
% are the symbolic relations shown in Table~\ref{tab:symbolic-relation-syntax},
enable the identification of the slicing seed $\textsf{userCity}$ at line 26 of Figure~\ref{fig:example}(a), and \textsf{CtrlDep} collects the expressions which are the control dependencies of $\textsf{userCity}$.
\end{example}

\begin{comment}
Similarly, we can introduce two additional neural relations, namely \text{XSSSrcExpr\_neural} and \text{XSSSinkExpr\_neural}, and customize the analysis policy of an intra-procedural XSS detection, which is shown in Figure~\ref{fig:xss-rules}.
In order to populate the relations \textsf{DataDep}, \text{XSSSrcExpr\_neural}, and \text{XSSSinkExpr\_neural}, the user instantiate neural relation constructors by specifying neural relation specifications, which will be demonstrated in~\cref{subsec:nrc}.


Leveraging these symbolic relations, the users can specify an analysis policy conforming to the syntax in Figure~\ref{fig:syntax} and introduce their own neural relations

Notably, the symbolic relations and neural relations essentially make up the extensional database in traditional Datalog engine. However, the difference is that neural relations can not be trivially populated. Due to the potential overhead of prompting, the population of neural relations can introduce much higher overhead than symbolic relations.
\end{comment}


\subsubsection{Neural Relation}

While symbolic relations effectively capture syntactic properties, many semantic properties, such as data dependencies, cannot be easily extracted through parsing alone. To address this, our analysis policy incorporates neural relations in the rules, enabling user-customized semantic analysis. 
% The key insight is that prompting LLMs offers a user-friendly interface for deriving semantic properties. 
By providing the definition of a semantic property along with several examples and the program to be analyzed, the desired semantic property can be obtained through few-shot CoT prompting, thereby populating the neural relations in Figure~\ref{fig:syntax}. We introduce the concept of \emph{neural relation specification} as follows to formulate how a user specifies a neural relation.

\begin{definition}(Neural Relation Specification)
	Given a neural relation, its neural relation specification is a pair of a natural language description $D$ and a set of examples $\mathcal{E}$. Here, the natural language description $D$ defines the desired semantic property. An example in $\mathcal{E}$ contains an example program $P_e$ and an explanation $E_e$ on the program property upon the example program $P_e$.
\end{definition}

\begin{example}
	\label{ex:nrs}
	For the analysis policy in Figure~\ref{fig:input}(a),
	we can provide the neural relation specification in Figure~\ref{fig:input}(b) for the neural relation \textsf{DataDep} so that the LLMs can produce all the tuples in \textsf{DataDep} depicting all the expressions with data dependencies.
	Similarly, the neural relations \textsf{XSSSrcNeural} and \textsf{XSSSinkNeural} shown in Figure~\ref{fig:xss-rules} depict the sources and sinks in the XSS bug detection, respectively,
    while
	the neural relation \textsf{TaintProp} captures intra-procedural taint flows.
	 \shi{put the materials into two examples, for fig 4 and fig 6, respectively?}\xz{you seem to assume that the LLM just magically derive all semantic properties. More indepth discussions such as how LLM can deal with complex semantic properties should be very helpful. Basically, complex aliasing relations can be prompted through LLM? Because LLM is able to derive transitive and complex relations (with degraded accuracy). I think you need to bring up the point that the neural relations only deal with primitive semantic relations and you rely on the datalog engine to derive further information. }
\end{example}


Intuitively, a neural relation specification formulates a skeleton that prompts LLMs to populate the corresponding neural relation. The supplied definition and examples can coach LLMs in deriving semantic properties from source code without compilation. More importantly, writing such specifications is both declarative and inductive, eliminating the need for users to modify compiler internals for customization. Hence, introducing such neural relation specifications can significantly improve the customizability of static analysis. \xz{I think some of the LLMSan idea for cross-checking can be mentioned/brought-in here because you seem not to mention how to validate results at all. I am sure that reviewers will ask you that kind of questions}




\subsection{Static Analysis via Analysis Policy Evaluation}
\label{subsec:pf}

%\shi{I suggest changing the title so that readers/reviewers can easily get what will be discussed in this section. Feel free to change it back if you do not like.}

Based on the pre-defined symbolic relations in Table~\ref{tab:symbolic-relation-syntax} and customized neural relations with their specifications,
% we can fully determine the semantics of an analysis policy specified by the users.
% Specifically, the symbolic relations can be generated by parsing the AST of the analyzed program,
% while the neural relations can be populated via few-shot CoT prompting with the guidance of the neural relation specifications.
% Eventually, 
we can derive the targeted program property by evaluating the analysis policy.
Thus, we reduce a static analysis problem to an analysis policy evaluation problem, formulated as follows.

\mybox{
Given a program $P$, an analysis policy $p$, and a set of neural relation specifications \emph{$\textsf{Specs}$},
we aim to derive all the tuples of the output relation $R^{*}$ in the analysis policy $p$,
which depicts the targeted program property of the program $P$.
}

Unlike traditional Datalog evaluation, evaluating an analysis policy in our problem exhibits two unique challenges,
which can significantly impact the effectiveness and efficiency of the analysis.
First, populating neural relations via prompting may introduce hallucinations, which cause the missing or wrong tuples in the neural relations,
further yielding the low precision and recall of the whole analysis.
Second, the evaluation of an analysis policy may require numerous prompting rounds, 
potentially consuming substantial token and time costs.
To achieve effective and efficient static analysis,
we need to address the above challenges in the analysis policy evaluation,
which will be detailed in~\cref{sec:approach}.
\shi{Previously, we discussed a few challenges related to hallucination in sec 2.2.2. Here, we start to discuss the challenges of datalog evaluation. Are they the same? We should find a way to state them uniformly and clearly. Otherwise, reviewers may be confused about what challenges we really address.}\wcp{revised}


\begin{comment}
However, populating neural relations with LLMs can still induce hallucinations,
potentially yielding low-quality analysis results. Also, each prompting round may have a non-trivial
time cost, which can become unacceptable when the number of prompting rounds is large.
\end{comment}















